ISTRBoost: Importance Sampling Transfer Regression using Boosting

Current Instance Transfer Learning (ITL) methodologies use domain adaptation and sub-space transformation to achieve successful transfer learning. However, these methodologies, in their processes, sometimes overfit on the target dataset or suffer from negative transfer if the test dataset has a high variance. Boosting methodologies have been shown to reduce the risk of overfitting by iteratively re-weighing instances with high-residual. However, this balance is usually achieved with parameter optimization, as well as reducing the skewness in weights produced due to the size of the source dataset. While the former can be achieved, the latter is more challenging and can lead to negative transfer. We introduce a simpler and more robust fix to this problem by building upon the popular boosting ITL regression methodology, two-stage TrAdaBoost.R2. Our methodology,~\us{}, is a boosting and random-forest based ensemble methodology that utilizes importance sampling to reduce the skewness due to the source dataset. We show that~\us{}~performs better than competitive transfer learning methodologies $63\%$ of the time. It also displays consistency in its performance over diverse datasets with varying complexities, as opposed to the sporadic results observed for other transfer learning methodologies.

==> header.tex <==
\usepackage{fixltx2e}
\usepackage{subcaption}
\usepackage{wrapfig}
\captionsetup[table]{skip=10pt}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
\usepackage[ruled, lined, linesnumbered, commentsnumbered, longend]{algorithm2e}

\newcommand{\ie}{\emph{i.e.},}
\newcommand{\eg}{\emph{e.g.},}
\newcommand{\etal}{\emph{et~al.}}
\newcommand{\sig}[1]{\ensuremath{\textrm{sig}(#1)}}

%% Uncomment these
\newcommand{\us}{\small\textsc{S-TrAdaBoost.R2}\normalsize}
\newcommand{\usas}{\small\textsc{S-TrAdaBoost.R2*}\normalsize}
\newcommand{\tradaR}{\small\textsc{TrAdaBoost.R2}\normalsize}
\newcommand{\adaR}{\small\textsc{AdaBoost.R2}\normalsize}
\newcommand{\ada}{\small\textsc{AdaBoost}\normalsize}
\newcommand{\trada}{\small\textsc{TrAdaBoost}\normalsize}
\newcommand{\ttradaR}{\small\textsc{two-stage TrAdaBoost.R2}\normalsize}
\newcommand{\adaRx}{\small\textsc{AdaBoost.R2X}\normalsize}
\newcommand{\gbr}{\small\textsc{Gradient Boosting}\normalsize}
\newcommand{\gbrx}{\small\textsc{Gradient BoostingX}\normalsize}
\newcommand{\kmmx}{\small\textsc{KMM.TL}\normalsize}
\newcommand{\kliepx}{\small\textsc{KLIEP.TL}\normalsize}
\newcommand{\iwkrrx}{\small\textsc{IW-KRR.TL}\normalsize}

\newenvironment{itemtight}{ 
 \begin{list}{$\bullet$\hfill}
  {\setlength{\parsep}{0ex}\setlength{\itemsep}{0ex}
   \setlength{\labelwidth}{0.10in}\setlength{\labelsep}{0.05in}
   \setlength{\leftmargin}{0.15in}\setlength{\rightmargin}{0.0in}
  }
}{
 \end{list}
} 


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


